Evaluation of microseismic motion at the KAGRA site based on ocean wave data

The microseismic motion, ambient ground vibration caused by ocean waves, affects ground-based gravitational wave detectors. In this study, characteristics of the ocean waves including seasonal variations and correlation coefficients were investigated for the significant wave heights at 13 coasts in Japan. The relationship between the ocean waves and the microseismic motion at the KAGRA site was also evaluated. As a result, it almost succeeded in explaining the microseismic motion at the KAGRA site by the principal components of the ocean wave data. One possible application of this study is microseismic forecasting, an example of which is also presented.

==> subsec4.1.tex <==
\subsection{Prediction of the ground motion with short period}
We also consider the prediction by using short period ground vibration data. 
Although KAGRA has already collected sufficient ground vibration data, for example, 
when selecting candidate sites for new gravitational wave detectors, 
it would be possible to shorten the site selection period if the effect of the ground vibration could be investigated over a short period of time. 

Figure \ref{fig:Prediction} and figure \ref{fig:PredRario} show the prediction of ground vibration by using wave height data of different periods.The figure on the left shows the prediction results using ground vibration data for January, and right figure shows the prediction results using data for one year.
Figure \ref{fig:Prediction} shows seismometer data on the horizontal axis, 
predictions on the vertical axis, and the number of data in the color bar. 
Figure \ref{fig:PredRario} changes the vertical axis in Figure \ref{fig:Prediction} to the difference between the predicted and measured values divided by the measured value.
In this figure, if the predicted value is close to the actual value, the value approaches 0. However, as the measured value increases, the value becomes smaller than 0.
Figure \ref{fig:HistCom} is a histogram for values of the ground vibration 
greater than 0.25$\mu m/s$ in Figure \ref{fig:PredRario}. 
The horizontal axis is the error from the measured value and the vertical axis is the number of data; 
the prediction for the January data has a mean value of 0.012 and a standard deviation of 0.316, 
while the prediction for the one-year data has a mean value of 0.033 and a standard deviation of 0.302. 
From figure \ref{fig:Prediction}, figure \ref{fig:PredRario} and figure \ref{fig:HistCom}, it can be seen that prediction with data for January has the same level of predicting accuracy as using data for one year in prediction using periods with large changes in wave height.

Figure \ref{fig:Mean_Sigma} shows the mean and standard deviation when predictions are made using data for each month. The same calculations as the standard deviations shown in figure \ref{fig:HistCom} are made for the prediction results for each month.
And, figure \ref{fig:CoefficientOfDetermination} shows the coefficient of determination when predictions are made using data for each month. 
Figure \ref{fig:Mean_Sigma} shows that from January to April and from October to December, the mean value is close to zero and the standard deviation is about the same as when one year of data is used.
On the other hand, it can be seen that the mean from May to September is heavily negatively biased. 
In other words, this indicates that predictions using data from the summer period or small value period will estimate smaller values than the actual values. 
The prediction for October is biased in the positive direction, but this may be due to the fact that the prediction is made using data for the period affected by typhoons, resulting in a larger estimate than the actual value. 
Figure \ref{fig:CoefficientOfDetermination} shows that the coefficients of determination for January through May, July, November, and December are about the same as when one year of data is used. 
On the other hand, the coefficients of determination were poor in the predictions for June, August, September, and October. 
Since the accuracy is high mainly in winter, when waves in the Sea of Japan develop, we believe that the accuracy of the prediction may be affected by the inclusion in the data used for the prediction of the period during which the characteristics of waves appear.
The results in Figures \ref{fig:Mean_Sigma} and \ref{fig:CoefficientOfDetermination} indicate that predictions using data from January through April, November, and December are as accurate as predictions using data from one year. 
On the other hand, predicting accuracy deteriorates when predictions are made using periods when the influence of waves is small, or when predictions are made using periods when typhoons have a strong influence.


\begin{figure}[ht]
    \begin{tabular}{cc}
      \begin{minipage}[t]{0.45\hsize}
        \centering
        \includegraphics[keepaspectratio, width=6.5cm]{fig/PredictionJan.pdf}
        \label{fig:PredictionJan}
      \end{minipage} &
      \begin{minipage}[t]{0.45\hsize}
        \centering
        \includegraphics[keepaspectratio, width=6.5cm]{fig/PredictionYear.pdf}
        \label{fig:PredictionYear}
      \end{minipage} \\
    \end{tabular}
    \caption{Comparison of predictions using January data and predictions using one year of data1. The left figure is scatterplot of prediction results using January data. The vertical axis is the predicted value. The right figure is scatterplot of prediction results using one year of data. The vertical axis is the predicted value.}
    \label{fig:Prediction}
\end{figure}
\begin{figure}[ht]
    \begin{tabular}{cc}
      \begin{minipage}[t]{0.45\hsize}
        \centering
        \includegraphics[keepaspectratio, width=6.5cm]{fig/PredRarioJan.pdf}
        \label{fig:PredRarioJan}
      \end{minipage} &
      \begin{minipage}[t]{0.45\hsize}
        \centering
        \includegraphics[keepaspectratio, width=6.5cm]{fig/PredRarioYear2.pdf}
        \label{fig:PredRarioYear}
      \end{minipage} \\
    \end{tabular}
    \caption{Comparison of predictions using January data and predictions using one year of data2. The left figure is scatterplot of prediction results using January data. The vertical axis shows the error from the actual measurements. The right figure is scatterplot of prediction results using one year of data. Vertical axis shows error from actual measurements.}
    \label{fig:PredRario}
\end{figure}


  
\begin{figure}[ht]
    \centering
    \includegraphics[clip,width=15cm]{fig/HistCom.pdf}
    \caption{Comparative histograms for January and year. The threshold is set to 0.25$\mu m/s$. The blue and orange vertical lines indicated deviations from the mean by a standard deviation, respectively.}
    \label{fig:HistCom}
\end{figure}


